Approximating CSPs with Outliers

Constraint satisfaction problems (CSPs) are ubiquitous in theoretical computer science. We study the problem of StrongCSPs, i.e. instances where a large induced sub-instance has a satisfying assignment. More formally, given a CSP instance $\Psi(V, E, [k], \{\Pi_{ij}\}_{(i,j) \in E})$ consisting of a set of vertices $V$, a set of edges $E$, alphabet $[k]$, a constraint $\Pi_{ij} \subset [k] \times [k]$ for each $(i,j) \in E$, the goal of this problem is to compute the largest subset $S \subseteq V$ such that the instance induced on $S$ has an assignment that satisfies all the constraints. In this paper, we study approximation algorithms for Unique Games and related problems under the StrongCSP framework when the underlying constraint graph satisfies mild expansion properties. In particular, we show that given a Strong Unique Games instance whose optimal solution $S^*$ is supported on a regular low threshold rank graph, there exists an algorithm that runs in time exponential in the threshold rank, and recovers a large satisfiable sub-instance whose size is independent on the label set size and maximum degree of the graph. Our algorithm combines the techniques of Barak-Raghavendra-Steurer (FOCS'11), Guruswami-Sinop (FOCS'11) with several new ideas and runs in time exponential in the threshold rank of the optimal set. A key component of our algorithm is a new threshold rank based spectral decomposition, which is used to compute a "large" induced subgraph of "small" threshold rank; our techniques build on the work of Oveis Gharan and Rezaei (SODA'17) and could be of independent interest.

==> header.tex <==
\newcommand{\card}[1]{\ensuremath{|#1|}}
\DeclareMathOperator*{\val}{val}
\DeclareMathOperator*{\var}{var}
\DeclareMathOperator*{\cl}{cl}
\DeclareMathOperator*{\opt}{OPT}
\DeclareMathOperator*{\disa}{disagr}
\DeclareMathOperator*{\rdisa}{rdisagr}
\DeclareMathOperator*{\lp}{LP}
\DeclareMathOperator*{\lpc}{\mathcal{L}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\polyloglog}{polyloglog}
\DeclareMathOperator*{\supp}{supp}
\DeclareMathOperator{\sos}{sos}
\DeclareMathOperator{\cli}{CLIQUE}
\DeclareMathOperator*{\maj}{Majority}
\DeclareMathOperator*{\unsat}{UNSAT}
\DeclareMathOperator*{\EX}{\mathbb{E}}
%\DeclareMathOperator*{\deg}{deg}
\newcommand{\etal}{\text{et al.}}
\newcommand{\etals}{\text{et al. }}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\tcW}{\widehat{\cW}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cX}{{\rm{X}}} % irit: I don't like the caligraphic X because it looks like a swastika and bad historical connotations. Can we find something else?
\newcommand{\cI}{\mathcal{I}}
%\newcommand{\cP}{\mathcal{P}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
%\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\tcS}{\widetilde{\cS}}
\newcommand{\tcT}{\widetilde{\cT}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\tGamma}{\tilde{\Gamma}}
\newcommand{\tG}{\tilde{G}}
\newcommand{\tV}{\tilde{V}}
\newcommand{\tE}{\tilde{E}}
\newcommand{\tw}{\tilde{w}}
\newcommand{\tC}{\tilde{C}}
\newcommand{\tO}{\tilde{O}}
\newcommand{\tcF}{\tilde{\cF}}
\newcommand{\tSigma}{\tilde{\Sigma}}
\newcommand{\ttau}{\tilde{\tau}}
\newcommand{\tP}{\tilde{P}}
\newcommand{\tS}{\tilde{S}}
\newcommand{\tU}{\tilde{U}}
\newcommand{\tu}{\tilde{u}}
\newcommand{\tv}{\tilde{v}}
\newcommand{\tcP}{\tilde{\cP}}
\newcommand{\tPhi}{\widetilde{\Phi}}
\newcommand{\x}{\times}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Fp}{\mathbb{F}_p}
\newcommand{\F}{\mathbb{F}_2}
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\scrA}{\mathscr{A}}
\newcommand{\scrP}{\mathscr{P}}
\newcommand{\Rz}{\mathbb{R}_{\geq 0}}
\newcommand{\ind}{\mathds{1}}
\newcommand{\vone}{\mathbf{1}}
\newcommand{\cost}{\cC}
\newcommand{\geqs}{\geqslant}
\newcommand{\leqs}{\leqslant}
%\renewcommand{\E}{\mathbb{E}}
\newcommand{\ow}{\overline{w}}
\newcommand{\f}{\frac}
\newcommand{\reg}{\text{reg}}
\newcommand{\greedy}{\text{greedy}}
\renewcommand{\bar}{\overline}
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\nullset}{\emptyset}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\DYES}{\mathcal{D}_{YES}}
\newcommand{\DNO}{\mathcal{D}_{NO}}
\newcommand{\YES}{{\sc YES}~}
\newcommand{\NO}{{\sc NO}~}
\newcommand{\loglog}{\log\log}
\renewcommand{\polylog}{\text{polylog}}
\renewcommand{\poly}{\text{poly}}
\newcommand{\psim}{\psi_{\text{maj}}}
\newcommand{\agr}{\text{agree}}
\newcommand{\napprox}{\not\approx}


==> partial-color.tex <==
\section{Partially $4$-coloring Partially $3$-colorable Graphs}				\label{sec:col}

In this section, we show how to compute a partial $4$-coloring of partially $3$-colorable low threshold rank graphs. The algorithm is almost similar to the one used for \stronguniquegames; the key differences are in the notion of threshold rank used for the analysis of the variance reduction step. As was shown in \cite{AG11}, the variance reduction step works in the case when the normalized adjacency matrix has a few large {\em negative} eigenvalues. Intuitively, this helps because here one wishes to make sure that vectors corresponding to neighboring vertices are as negatively correlated (i.e, far off) with each other as possible, since in any valid coloring, one has to assign distinct colors to neighboring vertices. 
We now state our result for the $3$-coloring problem, for $(\epsilon,\gamma)$-dense graphs.

\col*

\begin{algorithm}[ht!]				
	\SetAlgoLined
	\KwIn{A $(1-\delta)$-partially $3$-colorable graph $G = (V,E)$}
	Set parameter $R = Cr/\gamma$ and solve the following $R$-round Lasserre relaxation of $3$-Coloring SDP: 
	\begin{eqnarray*}
		& \sum_{i \in V} \left\langle v_{\{a\}\cup S,\{*\} \cup x_S},\vphi\right\rangle \leq \delta n \left\langle v_{S,x_S},\vphi \right\rangle  & \forall S \in \mathsmaller{{V \choose \leq r}}, x_S \in \{1,2,3,*\}^S \\
		& \left\langle v_{S,x_S},v_{T,\beta} \right\rangle = \left\langle v_{S',x_S'},v_{T',\beta'} \right\rangle & \forall S \cup T = S' \cup T' \\
		& \sum_{a \in [3]}\left\langle v_{(i,S,),(a,x_S)}, v_{(j,S),(a,x_S)} \right\rangle \leq 0 
		 &\forall \set{i,j} \in E, a \in \{1,2,3\} ,\\
		&													& \quad S \in \mathsmaller{{V \choose \leq R}}, x_S \in \{1,2,3,*\}^S
	\end{eqnarray*}\\
	Initialize 
	\[
		V_0 \gets V \qquad\qquad S_0 \gets \emptyset \qquad\qquad m \gets 0	\qquad {\sf Flag} \gets 0
	\]
	\While{$|V_m| \geq \epsilon|V|$ and $m \leq r$}
	{
	Compute 
	\[
	V_m = \left\{i \in V : \mu_{i,*|X_{S_m} \gets \alpha_m} \leq \gamma \mbox{ and }  \max_{a \in [3]} \mu_{i = a|X_{S_m} \gets \alpha_m} \leq \frac12 + \gamma \right\}
	\]
	Let $Q_m$ be the output of the $2$-approximation algorithm for vertex cover on $G[V_m]$\;
	\If{$|Q_m| \leq (\epsilon/5)n$}
	{
	Delete $Q_m$ from the graph, and for every $i \in V_m \setminus Q_m$ assign $\sigma(i) \gets 4$\;
 	Set ${\sf Flag} \gets 1$ and Break\;	
	}
	Choose $i \sim V \setminus S_m$ uniformly at random\;
	Sample $x_i \sim \mu_{i| X_{S_m} \gets \alpha_m}$\;
	Update $S_{m + 1} \gets S_m \cup \{i\}$ and $\alpha_{m + 1} \gets \alpha_m \circ x_i$;
	Set $m \gets m + 1$\;
	}
	Let $x_{S} := X_{S_m} \gets \alpha_m$ denote the final conditioning and compute set $V'$ as 
	\[
	V' = \left\{i \in V \setminus S \Big| \max_{a \in [3]} \mu_{i = a|x_S} > \frac12 + \gamma \right\} . \] 
	For every vertex $i \in V'$, assign $\sigma(i) \defeq \arg\max_{i \in [3]} \mu_{i,a|x_S,a \neq *}$\;
	\If{${\sf Flag} == 1$}
	{
	Output the set $V' \uplus (V_m \setminus Q_m) $ with coloring $\sigma$\;
	}
	\Else
	{
	Output the set $V' $ with coloring $\sigma$\;
	}
	\caption{Partial $3$-color}
	\label{alg:color}
\end{algorithm}


The algorithm for Theorem \ref{thm:thr-graph} is described in Algorithm \ref{alg:color}. For the analysis of the algorithm, we introduce some additional notation used in this section. For every subset $S$ of size at most $R$ and an assignment $\alpha \in \{1,2,3,*\}^S$, we can write $v_{S,\alpha} = \mu_{X_S = \alpha} \vphi + u_{S,\alpha}$, where $\mu_{X_S = \alpha} = \langle v_{S,\alpha},\vphi \rangle$ is interpreted as the probability of assigning color $\alpha$ to $S$ and $u_{S,\alpha}$ is the component of $v_{S,a}$ orthogonal to $\vphi$ . Furthermore, for a given vertex $i \in V$, we shall use $z_i$ to denote the concatenated vector $z_i:=(u_{i,1} u_{i,2} u_{i,3})$. Note that the definition of the $z_i$ vectors ignore the $X_i \gets *$ event. This is because (similar to \cite{AG11}), the $\{u_{i,a}\}_{a \in [3]}$ vectors are the ones responsible for the SDP solution approximately respecting the $3$-coloring constraints, and hence will result in large negative local correlation (see Lemma \ref{lem:loc-bound} for the formal argument).

We shall use $X_S$ and $x_S$ to differentiate between the random variable denoting the assignment to the subset of vertices in $S$ and the actual assignment itself. For a conditioning $X_S \gets x_S$ for some $x_S \in \{1,2,3,*\}^S$, we shall use $v_{T,\beta}|x_S, u_{T,\beta}|x_S$ and $z_{i}|x_S$ to be conditioned analogues of the $v_{T,\beta},u_{T,\beta}$ and $z_i$ vectors defined according to Proposition \ref{prop:las_cond}. As a first step, we begin by showing that feasibility of the SDP relaxation.

\begin{claim}
	The SDP relaxation in Algorithm \ref{alg:color} is feasible.
\end{claim}
\begin{proof}
	The proof of this is similar to that of Claim \ref{cl:sdp-bound}. Let $V_{\rm good}$ be the set of size at least $(1 - \delta)n$ such that the induced sub-graph $G[V_{\rm good}]$ is $3$-colorable, and Let $\sigma:V_{\rm good} \to \{1,2,3\}$ be the corresponding $3$-coloring.
	Now consider the following $1$-dimensional vector solution
	\[
	v_{i,a} = 
	\begin{cases}
	1 & \mbox{ if } i \in V_{\rm good}, \sigma(i) = a \\
	1 & \mbox{ if } i \notin V_{\rm good}, \sigma(i) = * \\
	0 & \mbox{ otherwise. } 
	\end{cases}
	\]
	Furthermore, we set $\vphi = 1$. As before, we extend it to a consistent $R$-local solution by defining $v_{S,\alpha} = \prod_{i \in S} v_{i,\alpha_i}$ (since $v_{i,a}$'s are scalars, the product operation is well defined). Now we proceed to verify that this is a feasible solution to the SDP.
	\begin{enumerate}
		\item Since $v_{i,a}$'s corresponding to an integral assignment, they satisfy all the Lasserre/SoS constraints.
		\item Since $|V \setminus V_{\rm good}| \leq \delta n$, for any subset $S$ and assignment $\alpha \in \{1,2,3\}^S$ we have 
		\[
		\sum_{i \in V} \left\langle v_{\{a\},\{*\} \cup \alpha},\vphi\right\rangle 
		=\sum_{i \in V} \mathbbm{1}(i \notin V_{\rm good}) \cdot \mathbb{1}(\sigma(S) = \alpha) = |V \setminus V_{\rm good}| \langle v_{S,\alpha},\vphi\rangle \leq \delta n\langle v_{S,\alpha},\vphi\rangle 	
		\]
	\item Finally, it is easy to see that no edge is labeled using $(a,a)$ for $a \in \{1,2,3\}$ and therefore the third constraint is satisfied trivially.
	\end{enumerate}
\end{proof} 
The next claim (similar to Lemma 4 from \cite{AG11}) shows that the algorithm returns a valid coloring.
\begin{claim}			\label{cl:col-feasible}
	The algorithm returns a valid $4$-coloring on the set of vertices it returns.
\end{claim}
\begin{proof}
	We begin by showing that the coloring $\sigma:V' \to [3]$ is always a valid $3$-coloring on $G[V']$. Fix an edge $\set{i,j} \in E[V']$ and for brevity let $a_i = \sigma(i),a_j = \sigma(j)$. Suppose for contradiction we have $a_i = a_j$. Then we have 
	\begin{align*}
	&\Pr\Big[X_i = a_i \wedge X_j = a_j \big| x_S\Big] \\
	&=  \Pr\Big[X_i = a_i \big| x_S\Big] + \Pr\Big[X_j = a_j \big| x_S\Big]  - \Pr\Big[X_i = a_i \vee X_j = a_j \big| x_S\Big] \\
	&\geq 2\cdot\left(\frac12 + 10\gamma\right)- 1 \geq 10\gamma .
	\end{align*} 
	On the other hand, from the SDP constraints we have 
	\[
	\Pr\Big[X_i = a_i \wedge X_j = a_j \big| x_S\Big]
	\leq 0 
	\]
	which contradicts the lower bound whenever $\gamma >0$. Therefore for any edge $\set{i,j} \in E[V']$ we must have $\sigma(i) \neq \sigma(j)$.
	
	Now to finish the proof, we consider two cases. Suppose ${\sf Flag} = 0$. Then the algorithm simply outputs $V'$ with the $3$-coloring, and hence we are done. Otherwise, if ${\sf Flag} = 1$, the {\em while loop} must have terminated inside the {\em if} block of the algorithm. In that case, observe that by definition $G[V_m \setminus Q_m]$ is an independent set, and therefore, they can all be assigned the color $4$. Since $\sigma$ only assigns colors $\{1,2,3\}$ in $G[V']$,  $\sigma$ is a valid $4$-coloring on $G[V' \cup (V_m \setminus Q_m)]$.
\end{proof}

Now we proceed to bound the size of the subset returned using the following two lemmas.

\begin{lemma}
	Suppose the while loop terminates inside the {\bf if} block. Then $|V' \cup (V_{m} \setminus Q_m)| \geq (1 - \delta/\gamma  -\epsilon/5)n$.	
\end{lemma}
\begin{proof}
	Clearly, by the termination condition we have $|Q_m | \leq (\epsilon/5) n$. Furthermore, note that under any conditioning $X_S \gets \alpha$, have 
	\[
	\Pr_{i \sim V}\left[\mu_{i = *| X_S \gets \alpha} \geq \gamma\right] \leq \delta/\gamma
	\]
	using Markov's inequality. Since the only vertices deleted here are the ones for the which the above event happens, and the ones from $Q_m$, the claim follows.
\end{proof}
	
\begin{lemma}		\label{lem:set-bound-col}
	Suppose the while loop does not terminate inside the {\bf if} block. Then with probability at least $0.9$ we have  $|V'| \geq (1 - \epsilon - \delta/\gamma)n$.
\end{lemma}

The above lemmas combined with Claim \ref{cl:col-feasible} completes the proof of Theorem \ref{thm:col}. In the remaining part of this section, we prove Lemma \ref{lem:set-bound-col}.

\subsection{Proof of Lemma \ref{lem:set-bound-col}}

The key technical challenge in proving Lemma \ref{lem:set-bound-col} would be to show that with good probability over the choice of the random conditioning, there are many choices of $i \in V$ for each of which there exists a color $\sigma(i) \in \{1,2,3\}$ which has conditional marginal probability (i.e, conditioned on the choice of $x_S$) of at least $\frac12 + \gamma$. This is again argued using a local-to-global correlation argument. For the rest of this section, for a conditioning $x_S$ (for some subset $S \subseteq V$), we shall say that a vertex $i \in V$ is {\em undetermined} if 
\[
\max_{a \in \{1,2,3\}} \Pr_{\mu_i| x_S} \Big[X_i = a \Big] < \frac12 + \gamma 
\]
Note that by definition, any vertex $i \in S$ is determined for any conditioning $x_S \in [3]^S$. We shall now state a sequence of lemmas which will lower bound the size of the subset $V'$. We begin by showing that if for a given conditioning $x_S \in \{1,2,3,*\}^S$, there exists a large fraction of vertices which are undetermined, then the corresponding $z_i$ vectors must have large average negative correlation (similar to Lemma 5 from \cite{AG11})
	\begin{lemma}			\label{lem:loc-bound}
		Fix an iteration $m$ such that $|V_m| \geq \epsilon n$ and the while loop does not terminate under the {\sf if} block. Let $S$ denote $S_m$ and $x_S$ denote the conditioning at iteration $m$. Then
		\[
		\Ex_{\set{i,j} \sim E} \left[\langle z_i|x_{S},z_j|x_S \rangle\right] \leq -\frac{\eta}{16} .
		\]
	\end{lemma}
	\begin{proof}
		The proof of the lemma is a combination of the proof of Lemma 5 from \cite{AG11} along with modifications to incorporate the $(\epsilon,\eta)$-density condition and the slack constraints involving the label `*'. We begin by observing that since the while loop does not terminate inside the {\em if} block, $G[V_m]$ does not admit a vertex cover of size at most $(\epsilon/10)n$. Since $G$ is $(\epsilon,\eta)$-dense, it follows that $|E[V_m]| \geq \eta|E|$. Fix an edge $\set{i,j} \in E[V_m]$. From the definition of $V_m$, we have $\mu_{i= *|x_S}, \mu_{j = *|x_S} \leq \gamma$, and therefore 
		\begin{equation}		\label{eq:eqn1}
		0 \geq \sum_{a \in [3]}\langle v_{i,a}|x_S,v_{j,a}|x_S \rangle = \sum_{a \in [3]} \mu_{i = a|x_S}\mu_{j = a|x_S} + \langle z_{i}|x_S, z_j|x_S \rangle
		\end{equation}
		Furthermore, since we have 
		\[ \sum_{a \in [3]} \mu_{i = a|x_S},\sum_{a \in [3]} \mu_{j = a|x_S} \geq 1 - \gamma, 
		\qquad \textrm{ and } \qquad 
		\mu_{i = a|x_S},\mu_{j = a|x_S} \leq 1/2 + \gamma, \]
		we have that 
		\begin{equation}		\label{eqn:corr-bd}
		\sum_{a \in [3]} \mu_{i = a|x_S}\mu_{j = a|x_S} \geq \frac15 
		\end{equation}
		
		This is due to the observation that the worst possible assignment of probability masses on $\{1,2,3\}$ are of the form $(1/2 - \gamma/2, 1/2-\gamma/2,0)$ and $(0, 1/2-\gamma/2, 1/2 - \gamma/2 )$ (this was established for the setting $\gamma = 0$ in~\cite{AG11}, see Proposition \ref{prop:2-point} for a elementary proof). Therefore, rearranging Eq. \ref{eq:eqn1} we get that $\langle z_{i}|x_S, z_j|x_S \rangle \leq - 1/8$. Define the set $T := \{i \in V| \mu_{i = *|x_S} \leq \gamma\}$. We can now bound the average local correlation as follows: 
		\begin{align*}
		&\Ex_{\set{i,j} \sim E} \left[\langle z_i|x_S, z_j|x_S\rangle\right] \\
		&\overset{1}{\leq} 2\Pr_{i \sim V} [ i \notin T] + 2\gamma \Pr_{\set{i,j} \sim E}[\set{i,j} \in E[T]\setminus E[V_m]]  - (1/8) \Pr_{\set{i,j} \sim V}[\set{i,j} \in E[V_m]] \\
		&\leq 2 \delta/\gamma + 2\gamma  - \eta/8  \leq - \eta/16.
		\end{align*}
		Here step $1$ is obtained by breaking the expectation conditioning whether (i) $\{i,j\} \notin T \times T$, or (ii) $\{i,j\} \in T \times (T \setminus V_m)$, or (iii) $\{i,j\} \in V_m \times V_m$. For the conditional expectation in (i), we trivially bound the correlation by $1$, for (ii) and (iii) we bound it by Eq. \ref{eq:eqn1} and \ref{eqn:corr-bd} respectively. The last inequality follows from our choice of parameters. 
	\end{proof}
	
	We now state a couple of lemmas which together imply that whenever the average negative correlation is large, conditioning reduces average variance. The first lemma lower bounds the decrease in the average variance on conditioning in terms of global correlation between the $z_i$-vectors.
	\begin{lemma}			\label{lem:var-bound}
		Given a set $S \subseteq V$ of size at most $R-2$ and assignment $x_S \in \{1,2,3,*\}^S$ we have 
		\[
		\Ex_{i \sim V} \Ex_{x_i \sim \mu_{i|x_S}} \Ex_{j \sim V} {\rm Var}\Big[X_j|x_S\Big] - {\rm Var}\Big[X_j|x_{S \cup \{i\}}\Big]
		\geq C_0 \Ex_{i,j \sim V} \Big[\left\langle z_i | x_S, z_j | x_S \right\rangle^2 \Big]
		\]
		for some absolute constant $C_0$.
		\end{lemma}
	\begin{proof}
	The proof almost follows by combining a couple of observations from \cite{AG11}, with minor changes accounting for the assignment $*$. Using the axioms of probability, Lemma 3 from \cite{AG11} establishes the inequality
	\begin{equation}					\label{eq:z-bound}
	\Ex_{i \sim V} \Ex_{x_i \sim \mu_{i|x_S}} \Ex_{j \sim V} \left[{\rm Var}\Big[X_j|x_S\Big] - {\rm Var}\Big[X_j|x_{S \cup \{i\}}\Big]\right]
	\geq \frac14 \Ex_{i,j \sim V} \Ex_{a,b \sim \{1,2,3,*\}} \Big[\left\langle u_{i,a} | x_S, u_{j,b} | x_S \right\rangle^2 \Big]
	\end{equation}
	On the other hand, using the definition of conditioned the $z_i$ vectors we know that 
	\begin{eqnarray*}
	\Ex_{i,j \sim V} \Big[\left\langle z_i | x_S, z_j | x_S \right\rangle^2 \Big]
	&=& \Ex_{i,j \sim V} \left[\left(\sum_{a \in [3]}\left\langle u_{i,a} | x_S, u_{j,a} | x_S \right\rangle\right)^2\right] \\
	&\leq& 3\Ex_{i,j \sim V} \left[\sum_{a \in [3]}\left\langle u_{i,a} | x_S, u_{j,a} | x_S \right\rangle^2\right] \\
	&\leq& 3\Ex_{i,j \sim V} \left[\sum_{a,b \in [3] \cup \{*\}}\left\langle u_{i,a} | x_S, u_{j,b} | x_S \right\rangle^2\right] \\
	&=& 48\Ex_{i,j \sim V}\Ex_{a,b \sim [3] \cup \{*\}} \left[\left\langle u_{i,a} | x_S, u_{j,b} | x_S \right\rangle^2\right] 
	\end{eqnarray*} 
	where the first inequality in the above steps is due to Cauchy-Schwarz, and the second inequality is due to the non-negativity of the additional square terms in the summation. Plugging in the above bound in the RHS of Eq. \ref{eq:z-bound} gives us the desired inequality. 
	\end{proof}
	
	The next lemma states that if the local negative correlation between the $z_i$ vectors is large, then the global correlation between the $z_i$ vectors is also large.
	\begin{restatable}{lem}{lemcolor}					\label{lem:loc-to-glob2}
		Let $S$,$x_S$ be as in Lemma \ref{lem:loc-bound}. Then
		\[
		\Ex_{i,j \sim V} \left[\left\langle z_i | x_S, z_j | x_S \right\rangle^2\right] \geq \frac{C \eta^2}{r}     
		\]
		where $r = \lrank{-1/16}(G)$.
	\end{restatable}
	The proof of the above lemma mainly follows from proof of Theorem 2 in \cite{AG11} with minor modifications to account for the almost $3$-colorability assumption in our setting. For completeness, we include a proof of it in Section \ref{sec:misc}. Now using the above lemmas we are now ready to prove the main lemma using which we can lower bound the size of the set $S$. We point out that the following lemma is a {\em one-shot} version of the iterative conditioning argument used in \cite{AG11}. While in their setting, conditioning would imply progress only when there are enough vertices that are undetermined, in our setting we exploit the guarantee of the $(\epsilon,\eta)$-density condition to argue that the randomly chosen set when built iteratively ensures that at each step, at least a constant fraction of undetermined vertices become determined. 
	
	\begin{lemma}			\label{lem:good-r}
	Suppose $R \geq C'\epsilon r/\eta^2$ for some large constant $C'>0$. Then 
	\[
	\Pr_{m \sim [R],S \sim V^m,x_S \sim \mu_S} \left[\Pr_{i \sim V}\left[\max_{a \in [3]}\mu_{i = a|x_S} \leq \frac12 + \gamma \right] \geq \epsilon \right]  \leq 0.1
	\]
	\end{lemma}


\begin{proof}	
	From the rounding algorithm we have 
	\begin{align*}
		& \E_S \E_{X_S}\Big[ \E_i {\rm Var}(X_i) - {\rm Var}(X_i|X_S) \Big]\\
		& = \E_S \E_{X_S} \E_i \left[\sum_{m \in [R]} {\rm Var}(X_i |X_{S_{m}}) - {\rm Var}(X_i |X_{S_{m + 1}}) \right] \tag{Telecsoping sum}\\
		& = \sum_{m \in [R]} \E_{S \sim V^m} \E_{X_S} \E_i \E_{X_j} 
		\Big[{\rm Var}(X_i |X_{S}) - {\rm Var}(X_i |X_{S \cup \{j\}}) \Big] \\
	& \geq \sum_{m \in [R]} \E_{S \sim V^m,x_S \sim \mu_S} \E_{p,q \sim V} \Big[\langle z_p|x_S, z_q|x_S \rangle^2\Big] 
	\tag{Lemma \ref{lem:var-bound}}\\
	&{\geq} \frac{C \epsilon\eta^2}{r}\sum_{m \in [R]} \E_{S \sim V^m,x_S, \sim \mu_S}\mathbb{I}\left(\left|\E_{p,q \sim V} \langle z_p | x_S, z_q| x_S \rangle \right| \geq \frac{C \eta^2}{r} \right) \\
	\tag{{\rm Lemma}~\ref{lem:loc-to-glob2}}	
	&{\geq} \frac{C \epsilon\eta^2}{r}\sum_{m \in [R]} \E_{S \sim V^m,x_S, \sim \mu_S}\mathbb{I}\left(\left|\E_{(p,q) \sim E} \langle z_p | x_S, z_q| x_S \rangle \right| \geq \frac{\eta}{16} \right) \\
	& = \frac{C \epsilon\eta^2 R}{r}\Pr_{m \sim [R], S \sim V^m,x_S \sim \mu_S} \left[\left|\E_{(p,q) \sim E} \langle z_p|x_S, z_q|x_S \rangle \right| \geq \frac{\eta}{16} \right]  
	 \tag{Since $m \sim {\rm unif}(R)$}\\
	& \geq \frac{C \epsilon \eta^2 R}{r}\Pr_{m \sim [R], S \sim V^m,x_S \sim \mu_S} \left[\Pr_{i \sim V}\left[\max_{a \in [3]}\mu_{i = a|x_S} \leq \frac12 + \gamma \right] \geq \epsilon\right] \tag{Lemma \ref{lem:loc-bound}}
	\end{align*}
	Since the LHS in the above sequence of equations can be at most $1$, rearranging we get that 
	\begin{align*}
			\Pr_{m \sim [R],S \sim V^m,x_S \sim \mu_S}\left[\Pr_{i \sim V}\left[\max_{a \in [3]}\mu_{i = a|x_S} \leq \frac12 + \gamma \right] \geq \epsilon \right] \leq \frac{r}{C\eta^2 R} < 0.9
	\end{align*}
	where the last inequality follows from our choice of $R$.
			
\end{proof}
	
Now we prove Lemma \ref{lem:set-bound-col}.

\begin{proof}[Proof of Lemma \ref{lem:set-bound-col}]
From the above lemma we know that with probability at least $0.9$ over the choice of $m,S,x_S$, we have 
\[
\Pr_{i \sim V}\left[\max_{a \in [3]}\mu_{i = a|x_S} \leq \frac12 + \gamma \right] \geq \epsilon .
\]
Furthermore, since $\mu_S(X_S) \neq 0$, from the SDP constraints, we also have 
\[
\sum_{i \in V} \mu_{i = *|x_S} \leq \delta n
\] 
	which implies that for at least $(1 - \delta/\gamma)$-fraction of vertices we have $\mu_{i = *|x_S} \leq \gamma$. Therefore by a union bound we have $|V'| \geq (1 - \delta/\gamma - \epsilon)n$.
\end{proof}


==> robust-brs.tex <==
	\section{Finding Good Assignments in Vertex Induced CSPs}				\label{sec:robust-brs}
	
	\snote{Need to expand before the thm statement}
	In this section, we show that the BRS algorithm can be extended to the setting where the goal is to find a large vertex induced sub-graph on which most of the constraints are satisfied. The following theorem gives us the guarantees for this setting:
	
	\begin{theorem}						\label{thm:robust-brs}
	Let ${\Psi}(V,E,[k],\{\Pi_{(i,j)}\}_{(i,j) \in E})$ be a $2$-CSP on $n$-vertices such that there exists $V_{\rm good} \subset V$ of size $\epsilon n$ and a labeling which satisfies $\gamma$-fraction of edges in $E[V_{\rm good}]$. Then there exists a randomized algorithm  which runs in time $n^{{\rm rank}_{\epsilon/k^2}(G)/{\poly(\epsilon)}}$ and with probability at least $1 - e^{-\delta^2\epsilon n/4}$, outputs a set $V \subset V$ of size $(1 \pm \delta)\epsilon n$, and a labeling $\sigma:V' \mapsto [k]$ which satsifies at least $|E[V_{\rm good}]|/|E| - \epsilon$-fraction of edges in $\Psi$.
	\end{theorem}
	
	\section{Algorithm for Theorem \ref{thm:robust-brs} }
	
	
	\begin{algorithm}
		\SetAlgoLined
		\KwIn{A $2$-CSP ${\Psi}(V,E,[k],\{\Pi_{(i,j)}\}_{(i,j) \in E})$, and deletion parameter $\gamma \in (0,1)$}.
		Solve the following SheraliAdams relaxation for Unique Games
		\begin{eqnarray*}
			\text{min}  &  \frac{1}{|E|}\sum_{(i,j) \in E} \sum_{(a,b) \in \Pi_{(i,j)}} \langle v_{i,a},v_{j,b} \rangle  & \\
			\text{s.t.}& \sum_{i \in V} \left\|v_{\{a\}\cup S,\{i\} \cup \alpha}\right\|^2 = \epsilon n \left\|v_{S,\alpha}\right\|^2  & \forall S \in \mathsmaller{{V \choose \leq r}}, \alpha \in [k]^S \\
			& \left\langle v_{S,\alpha},v_{T,\beta} \right \rangle = \Pr\left[X_S = \alpha, X_T = \beta \right]  & \forall S \in \mathsmaller{{V \choose \leq r}}, \alpha \in [k]^S \\
		\end{eqnarray*}\\
		\nonl
		{\bf Rounding}:\\ 
		Sample $m \sim [r]$, $S \sim V^m$ and an assignment $X_S \sim \mu_S$\;
		For every $i \in V \setminus$, sample $X_i \sim \mu_{i}| X_S$.\;
		Delete vertices $\{i \in V | X'_{i} = k+1\}$.
		\caption{Robust BRS}
	\end{algorithm}
	
	The following claim lower bounds the SDP optimal.
	
	\begin{lemma}
		The SDP optimal is at least $\gamma|E_{\rm good}|/|E|$.
	\end{lemma}
	
	\begin{proof}
	Let $\sigma:V_{\rm good} \mapsto [k]$ be the partial labeling which satisfies all the induced constraints in $\cG[V_{\rm good}]$. Consider the following one dimensional solution.
	\[
	v_{i,a} = 
	\begin{cases}
	1 & \mbox{ if } i \in V_{\rm good}, a = \sigma(i) \\
	1 & \mbox{ if } i \notin V_{\rm good}, a = k+1 \\
	0 & \mbox{ otherwise } 
	\end{cases}
	\] 
	Furthermore, for every $S \in {V\choose \leq r}$ and assignment $\alpha \in [k+1]^S$, we define $v_{S,\alpha} = \prod_{i \in S} u_{i,\alpha(i)}$. Then using arguments identical to Claim \ref{cl:sdp-bound} it can be shown that this is indeed a feasible solution. Now we lower bound the objective. Consider any edge $(i,j) \in E[V_{\rm good}]$. Then by construction we must have $v_{i,\sigma(i)} = v_{j,\sigma(j)} = 1$. Using this observation we can lower bound the objective as 
	\begin{align*}
	\frac{1}{|E|}\sum_{(i,j) \in E} \sum_{(a,b) \in \Pi_{(i,j)}} \langle v_{(i,a)},v_{(j,b)} \rangle 
	\geq \frac{1}{|E|}\sum_{(i,j) \in E[V_{\rm good}]} v_{i,\sigma(i)}v_{j,\sigma(j)}
	\geq \frac{\gamma |E[V_{\rm good}]|}{|E|}
	\end{align*}
	
	\end{proof}
	
	
	\subsection{Guarantees of the Rounding Step}
	
	First we recall the following key lemma from BRS which would directly give us the guarantees of the rounding algorithm.
	
	\begin{theorem}
		Let $X_1,\ldots,X_n$ be the $r$-local random variables and $X'_1,\ldots,X'_n$ be the assignments produced by the rounding step of the algorithm (including those which vertices which are labeled $k+1$.) of the algorithm. Then for $r \geq O(k/\epsilon^4){\rm rank}_{\Omega(\epsilon/k)^2}(G)$ we have $\Ex_{(i,j) \sim E} \|\{X_iX_j\} - \{X'_iX'_j\} \|_1 \leq \epsilon$
	\end{theorem}
	
	Using the above theorem we get that 
	
	\begin{eqnarray*}
	\Pr_{(i,j) \sim E}\Big[\{X'_i,X'_j\} \in \Pi_{(i,j)}\Big] 
	&\geq& \Pr_{(i,j) \sim E}\Big[\{X'_i,X'_j\} \in \Pi_{(i,j)}\Big] - \Ex_{(i,j) \sim E} \|\{X_iX_j\} - \{X'_iX'_j\} \|_1 \\
	&\geq& \frac{\gamma|E_{\rm good}|}{|E|} - \epsilon\\
	\end{eqnarray*}
	
	Now we use the cardinality constraints to bound the number of vertices thrown away during the deletion step. Since the assignment $x_S$ was sampled from the $r$-local distribution $\mu_S$, it follows that $\Pr_{\mu_S}\Big[X_S = x_S\Big] = \left\| v_{S,\alpha}\right\|^2 > 0$. Now the global cardinality constraint $\sum_{i \in V} \left\|v_{\{i\} \cup S, \{k+1\} \cup \alpha} \right\|^2 \leq \epsilon n \left\|v_{S,x_S}\right\|^2$ can be reinterpreted as 
	\[
	\sum_{i \in V}\Pr\left[X_{i} = k+1 \Big| X_S = x_S\right] = \epsilon n
	\]
	Since conditioned on the choice of the seed set $S$ and the corresponding assignment $X_S$, the labelings of the vertices are independent, using Chernoff bound, with probability at least $1 - e^{-\gamma^2 \epsilon n}$, the number of vertices discarded is within $(1 \pm \gamma)\epsilon n$. Finally, observe that the subset of edges satisfied by the labeling output by the algorithm are in turn a subset of edges whose both end points are labeled from $[k]$. Therefore the deletion step does not affect the number of edges satisfied by labeling output by the algorithm. This completes the proof of Theorem \ref{thm:robust-brs}.
	
